Variance Alignment Score: A Simple But Tough-to-Beat Data Selection Method for Multimodal Contrastive Learning

In recent years, data selection has emerged as a core issue for large-scale visual-language model pretraining, especially on noisy web-curated datasets. One widely adopted strategy assigns quality scores such as CLIP similarity for each sample and retains the data pairs with the highest scores. However, these approaches are agnostic of data distribution and always fail to select the most informative samples. To solve this problem, we propose a simple yet theoretically principled metric named Variance Alignment Score (VAS), which has the form $\langle \Sigma_{\text{test}}, \Sigma_i\rangle$. Here, $\Sigma_{\text{test}}$ represents the target (cross-)covariance matrix we aim to align, potentially based on prior knowledge, while $\Sigma_i$ denotes the tensor product of single or multi-modal representations for the $i$-th sample. We further design a new data selection method that maximizes the total VAS. We provide theoretical analysis in a simplified setting to demonstrate the theoretical advantage of VAS over random or other existing data selection. Experimentally, applying VAS and CLIP scores together can outperform baselines by a margin of $1.3\%$ average on 38 evaluation sets for noisy dataset DataComp and $2.5\%$ on VTAB for high-quality dataset CC12M. Additionally, our ablation study also shows visual features are better than text for calculating VAS, and the related classical experimental design methods may fail under this context.

==> theory_archive.tex <==
\section{Theoretical interpretation}\label{sec:theory}
In this section, we give a theoretical justification on the second phase \yifang{right word ?} of our proposed strategy under the linear model assumptions when their is no corrupted or contaminated samples (e.g. low quality image, mismatched text) 

\subsection{Theoretical setup}
We give a rigorous theoretical interpretation on our learning problem as follows.

\paragraph{Training data generation}
For any $\vx^{v}, \vx^{l} \in \R^d$ observable image and text training pairs, we define $\vz^{v}, \vz^{l}$ to be the corresponding latent vectors which contains all the information we cared about. Similar to previous theoretical work \yifang{cite},
each pair of $(\vz_v,\vz_l)$ is an independent zero-mean sub-gaussian vector satisfies
\begin{align*}
    & \text{Cov}(\vz_v,\vz_l) 
    = \E_{\vz_v,\vz_l \sim \gD_\text{train}} \left[\vz_v \vz_l^\top\right]
    = \Gamma_\text{train},
    & \|\vz_{vl}\| = 1
\end{align*}
and $\vx^{vl}$ is generated based on a linear model that
\begin{align*}
    \vx^{vl} = G^*_{vl} \vz^{vl} + \vxi^{vl}.
\end{align*}
Here $G^*_l \in O_{d\times r}$ is the ground truth representation that maps from the latent vector space to the signal part of the input space, and $\xi^{vl} \sim \mathcal{N}(0, \sigma_{\xi}^2I_d)$ are \textit{i.i.d.} random noise, with $\sigma_{\xi} \ll 1$. 
For $n$ \textit{i.i.d.} samples, we denote $X^{vl} = (\vx^{vl}_1,\ldots, \vx^{vl}_n)^\top \in \R^{n \times d}$, $Z^{vl} := (\vz_1^{vl}, \ldots, \vz_n^{vl})^\top \in \R^{n \times r}$ 
and $\Xi^{vl} := (\vxi^{vl}_1,\ldots,\vxi^{vl}_n)^\top \in \R^{n \times d}$ to be the stacked matrix of inputs, embeddings and noise. 


\paragraph{Test data generation}
For any zero-shot downstream task, we assume it share the same linear representation and noise as train set. But the distribution of zero-mean normalized subgaussian latent vectors $\vz^{vl}$ might be different. That is, the cross-covariance $\Gamma_\text{test}$ does not necessary equal to $\Gamma_\text{train}$. We will discuss the impact of different distribution in the theorem section. 


% \paragraph{CLIP embedding model as teacher} Unlike classical data selection problem where we can only observe $x$ (i.e image, text), here we have a teacher model $\bar{G}_{vl}$, whose generated clip embedding can partially recover the ground truth hidden vector $\vz^{vl}$ with error $\epsilon_{vl}$,
% \begin{align*}
%     \E_{\vz^{vl}, \vx^{vl} \sim \gD_\text{train}} \langle \bar{G}_{vl}\vx^{vl}, \vz^{vl} \rangle \geq 1-\epsilon_{vl}
% \end{align*}
% \yifang{TODO: norm matters if choose 1}
% where $\gD_\text{train}$ is the join training distribution as described in the training data generation process. When $\bar{G}_{vl} = \bar{G}_{vl}^*$, the clip embedding is equivalent to hidden vector. 
% \yifang{Expectation is not strong enough.. maybe need to define over any $|S|$ sampling}

\paragraph{CLIP embedding model as teacher} Unlike classical data selection problem where we can only observe $x$ (i.e image, text), here we have a teacher model $\bar{G}_{vl}$, whose generated clip embedding can partially recover the ground truth hidden vector $\vz^{vl}$ with error. 

Formally, we say teacher has $\epsilon_{v}^n$ error if for all possible $n$ budget subet $S \subset D_\text{train}$,
\begin{align*}
    \frac{1}{|S|} \left\| \sum_{\vx_{vl} \in S} \bar{G}_v^\top \vx_v \vx_v^\top \Bar{G}_v - \sum_{\vx_{vl} \in S} \vz_v \vz_v^\top \right\|_* \leq \epsilon_{v}^n
\end{align*}
the same notation applies for language modal. In addition, we say teacher has $\epsilon_{v*l}^n$ cross modal error
\begin{align*}
   \frac{1}{n}\| \sum_{\vx_{vl} \in S} \bar{G}_v^\top \vx_v \vx_l^\top \Bar{G}_l - \sum_{\vx_{vl} \in S} \vz_v \vz_l^\top \|_*  \leq \epsilon_{v*l}^n
\end{align*}
When all $\epsilon_v^n, \epsilon_l^n, \epsilon_{v*l}^n \to 0$ , then the teacher is strong for both modal. But it might also be possible that only one modal, for example, visual is strong. That is $\epsilon_v^n \to 0,  \epsilon_l^n, \epsilon_{v*l}^n \gg \epsilon_v^n$.
\footnote{It is possible to represent $\epsilon_{v*l}^n$ using $\epsilon_v^n, \epsilon_l^n$. However, our primary objective in this section is to conceptually interpret our empirical results. Therefore, we will maintain this simpler version for ease of understanding.}




\paragraph{Model and training}
According to Lemma 4.1 in \cite{nakada2023understanding}, using the CLIP loss to optimize the linear model has approximately the same training dynamics as using the regularized linear loss. Therefore, here we assume that we are learning $G_v, G_l$ by maximizing the clip score gap between same-sample pairs and the contrastive pairs, plus the some regularization, 
\begin{align*}\label{eq:linearloss}
    & \min_{G_v, G_l} \gL_S (G_v, G_l) \\
    & := \min_{G_v, G_l} \frac{\sum_{i \in S} \sum_{j \in S \setminus \{i\}}(s_{ij} - s_{ii})}{n(n-1)} 
    + R(G_v, G_l) \\
    & = \min_{G_v, G_l} \frac{\sum_{i \in S} \sum_{j \in S}(s_{ij} - s_{ii})}{n(n-1)} 
    + R(G_v, G_l)
\end{align*}
where  $s_{ij} := \langle  G_v^\top \vx^v_i, G_l^\top \vx^l_j \rangle$ and $\gS$ is the $n$ size dataset after filtering. Notice here we abuse notation a little bit between indices $i,j$ and the actual sample $\vx^{vl}_i$. This format was also used in \yifang{cite}.

\paragraph{Goal and metric}
Under the same principle as our training loss function, we measure the performance of any learnt $G_v, G_l$ on some downstream task with distribution $\gD_\text{test}$ as test loss $\gL_{\text{test}} (G_v, G_l):=$
\begin{align*}
     \E_{\substack{\vx_{vl}\sim \gD_\text{test}\\\vx_{vl}' \sim \gD_\text{test}}} (\langle G_v^\top\vx_v, G_l^\top\vx_l'\rangle- \langle G_v^\top\vx_v, G_l^\top\vx_l\rangle) 
\end{align*}
% Here $ \gD_\text{test}^\epsilon$ denotes the discretized $\epsilon$-covering of continuous distribution  $ \gD_\text{test}$. 
% \yifang{TODO: Simon can you check if this notation is right ? or can we just use $\E_{\vx_{vl} \sim \gD_\text{test}} \E_{\vx_{vl}' \sim \gD_\text{test}}$}
\yifang{Double check if this is true}
Therefore let $\hat{G}_{vl}$ be the learnt representation from our selected subset $S$ and the $G_{vl}^{\text{random}}$ be the one from a random sampled subset under the same budget, our goal is to maximize
\begin{align*}
    \Delta(S) = \gL_\text{test}(\hat{G}_{vl}^{\text{random}}) - \gL_\text{test}(\hat{G}_{vl})
\end{align*}



\subsection{Generalization guarantees}
\yifang{Rewriting the whole structure....}



Based on the previous setting, we provide a theoretical guarantees in this section and discuss their connection to the actual algorithm we implemented in \yifang{cite}. We postpone our proof into Appendix~\ref{app: proof}.

Here we decompose the results into three items. The best possible improvement term stands for the for the optimal subset selection if we know the test distribution $\Gamma_{\text{test}}$ in advance, and the error from noise terms stands for the estimation error under any fixed budget $|S|$. Both of term characterize the natural hardness of the problem that it inevitable. 

\begin{theorem}[A simplified version of test loss]
\label{them: simplified test loss}
    Under the assumption that both $\vz_{vl}, \xi_{vl}$ is zero-mean, maximizing the clip score gap is equivalent to maximize the clip score of the same sample. 
     \begin{align*}
         \gL_{\text{test}} (G_v, G_l):= - \E_{\vx_{vl} \sim \gD_\text{test}}\langle G_v^\top\vx_v, G_l^\top \vx_l \rangle
     \end{align*}
\end{theorem}
\yifang{Maybe add some discussion say if the test data are high quality, then $\hat{G} = G^*$ is the best thing we could get. Otherwise, recovering $G^*$ might not be the best option. So we should use contrastive learning instead of directly do supervised learning on the teacher clip model.}

The improvement $\Delta(S) > 0$ is not always possible. We first characterize the hardness of the problem by decomposing $\Delta(S)$ into different sources.
\begin{lemma}[Hardness of the problem]
\label{lem: hardness}
    \yifang{With high prob?}, the improvement of our strategy compared to randomness sampling as 
    \begin{align*}
        &\Delta(S) 
        \geq \underbrace{\Tr \left( \Gamma_{\text{test}}(\Gamma_S - \Gamma_{\text{best}}) \right) }_{\text{err from our strategy} < 0} 
         + \text{hardness} \\
        & \text{hardness}:= \underbrace{\Tr \left( \Gamma_{\text{test}}(\Gamma_{\text{best}} - \Gamma_{\text{train}}) \right) }_{\text{best possible improvement}}
            - \underbrace{\text{\yifang{TODO}}}_{\text{err from noise}}
    \end{align*}
    where $\Gamma_S = \frac{1}{|S|}\sum_{\vz_{vl} \in S} \vz_v \vz_l^\top$ is the variance of chosen subset $S$ and $\Gamma_\text{best}$ is the variance best subset we could choose under the same budget. Formally, it is defined as: 
    \begin{align*}
        & \Gamma_\text{best} = \argmax_{\Gamma} \mathrm{tr\left( \Gamma_{\text{test}}\Gamma \right)} \\
        \text{s.t.} \quad 
        & \Gamma = \frac{1}{|S'|}\sum_{\vz_{vl} \in S'} \vz_v \vz_l^\top,
          S' \subset D_{train}, |S'| = |S|
    \end{align*}
The random sampling is unbeatable when 
$\text{hardness}< 0$
\end{lemma}

\begin{proof} 
(Sketch version)\\
\textbf{Step 1: Simplified the loss} 

    
\end{proof}
Here we decompose the results into three items. The best possible improvement term stands for the for the optimal subset selection if we know the test distribution $\Gamma_{\text{test}}$ in advance, and the error from noise terms stands for the estimation error under any fixed budget $|S|$. Both of term characterize the natural hardness of the problem that it inevitable. 



\begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\begin{subfigure}
	\centering
\includegraphics[width=\columnwidth]{fig/vas_cs_f0.451.png}
\end{subfigure}
\begin{subfigure}
	\centering
\includegraphics[width=\columnwidth]{fig/vas_cs_f0.451_text.png}
\end{subfigure}
% \vskip -0.2in
% \centerline{\includegraphics[width=\columnwidth]{Figures/heatmap_L1toL2_final_20.0.pdf}}
\caption{Image features are more concentrated than text features.\yiping{Should I add this kind of pic here? Just draft now.}} \yifang{What conclusion do you want to show ?}
\label{fig:img_txt}
\end{center}
\vskip -0.2in
\end{figure*}


Therefore, we should focus on the term `` error from our strategy". Such error mainly comes from (1) The unknown test distribution shift from training. (2) The unobservable ground truth $\Gamma_S$ as shown below. To tackle error (1), we assume some prior knowledge on test by using the proxy test variance $\bar{\Gamma}_{\text{test}}$. \yifang{TODO: say more} To tackle the error (2), we propose two solutions with theoretical interpretation as below. Based on the theoretical interpretation, we should choose different strategy based on the property of clip score.
\begin{align*}
    & S_{\text{Option 1}} = \argmax_{S} \Tr\left(\bar{\Gamma}_{\text{test}} (\sum_{\vx_{vl} \in S} \bar{G}_v^\top \vx_v \vx_l^\top \Bar{G}_l) \right)  \\
    &  S_{\text{Option 2}} = \argmax_{S} \Tr\left(\bar{\Gamma}_{\text{test}} (\sum_{\vx_{vl} \in S} \bar{G}_v^\top \vx_v \vx_v^\top \Bar{G}_v) \right)
\end{align*}


\begin{theorem}[Main]
\label{them: main}
    \begin{align*}
       \Delta(S)
        & \geq \text{hardness} -  \|\bar{\Gamma}_{\text{test}} - \Gamma_{\text{test}} \| \|\Gamma_S - \Gamma_{\text{best}}\| \\
        & \quad - 
        \begin{cases}
            \epsilon_{v * l}^S  \quad \text{(Option 1)} \\
            \epsilon_v^S +  \frac{1}{|S|}\| \sum_{\vx_{vl} \in S} \vz_v \vz_v^\top -  \Gamma_S\|_* \quad \text{(Option 2)}
        \end{cases}
    \end{align*}
\end{theorem}



\yifang{TODO: add discussion of $\bar{\Gamma}_{\text{test}}$}
It is easy to see that, when $\epsilon_l$ is large \yifang{More specific ?}, as shown in \yifang{Empirical evidence}, using image focused filtering is a better.





\iffalse
Now we are ready to show the main advantage of our strategy compared to the random sampling. We start with the case that teacher model can recover both $\vz_v,\vz_l$ with low error $\epsilon_{vl} \to 0$ in Theorem~\ref{them: main strong teacher}. In this case, we shall use clip embedding form both image and text. Nevertheless, our empirical result \yifang{cite} shows that using clip embedding from both modal performs much worse than using image embedding only. We further interpret this phenomena in Theorem~\ref{them: main weak teacher}.

\begin{theorem}[Results under a strong teacher]
\label{them: main strong teacher}
    Let $\hat{G}_{vl}$ be the learnt representation from our selected subset $S$ and the $G_{vl}^{\text{random}}$ be the one from a random sampled subset under the same budget. We have that, \yifang{with high prob?}
    \begin{align*}
        &\gL(\hat{G}_{vl}^{\text{random}}) - \gL(\hat{G}_{vl}) \\
        &\geq \underbrace{\Tr \left( \Gamma_{\text{test}}(\Gamma_{\text{best}} - \Gamma_{\text{train}}) \right) }_{\text{best possible improvement}}
            + \underbrace{\Tr \left( \Gamma_{\text{test}}(\Gamma_S - \Gamma_{\text{best}}) \right) }_{\text{err from test distribution shits}} \\
        &\quad - \underbrace{\text{\yifang{TODO}}}_{\text{err from noise}} 
          - \underbrace{\text{\yifang{TODO}}}_{\text{err from teacher model}}
    \end{align*}
    where $\Gamma_S = \frac{1}{|S|}\sum_{\vz_{vl} \in S} \vz_v \vz_l^\top$ is the variance of chosen subset $S$ and $\Gamma_\text{best}$ is the variance best subset we could choose under the same budget. Formally, it is defined as: 
    \begin{align*}
        & \Gamma_\text{best} = \argmax_{\Gamma} \mathrm{tr\left( \Gamma_{\text{test}}\Gamma \right)} \\
        \text{s.t.} \quad 
        & \Gamma = \frac{1}{|S'|}\sum_{\vz_{vl} \in S'} \vz_v \vz_l^\top,
          S' \subset D_{train}, |S'| = |S|
    \end{align*}
\end{theorem}

\paragraph{Discussion} 
\yifang{How test distribution affect}

\yifang{How quality $\text{Trace}(\Gamma)$ affect}

\yifang{Budget lower bound}

Above result will become meaningless when $\epsilon_l$ becomes larger. Fortunately, we are able to \textit{largely} reduce the error from teacher model in the sacrifice of a slightly increased error from test distribution shifts.

\begin{theorem}[Results under weak language modal teacher (Main)]
\label{them: main weak teacher}
    
\end{theorem}



\yifang{===== Below TODO ======}

Following \cite{nakada2023understanding, ji2023power}, we choose $R(G_1, G_2) = (\rho/2)\|G_1G_2^\top\|_F^2$ for some $\rho > 0$, which allows us to use Eckart-Young-Mirsky theorem [XXX] (Details in Appendix XXX) directly, and we can obtain the following closed-form solution
\begin{lemma}[Informal]\label{lemma:EYM}
    Let
    \begin{equation}
        \hat G_1, \hat G_2 = \arg \min_{G_1, G_2 \in \R^{d\times r}}\mathcal{L}(G_1,G_2)
    \end{equation}
    Then we have
    \begin{equation}
        \hat G_1 \hat G_2^\top = \frac{n}{\rho(n-1)}G_1^*V \cdot\Gamma\cdot V^\top (G_2^*)^\top + \text{noise}
    \end{equation}
    where
    \begin{equation}
        \Gamma :=\frac{1}{n}\sum_{l=1}^n\vy_i^{(1)}(\vy_{i}^{(2)})^\top
    \end{equation}
\end{lemma}

So the key points for improving the generalization error of $\hat G_1 \hat G_2^\top$ is to obtain benign $\Gamma$. If for any data point, $\vy^{(1)}$ aligns with $\vy^{(2)}$ well, then $\Gamma$ can be well diagonal and the generalization error is low. However, in the large scale training scenario of image-text foundation models, the data are always curated from web and thus low-qualitied, so the unfiltered dataset will result in non-diagonal terms in $\Gamma$ and performs badly. To formalize the context, we define:

\begin{definition}[Excess Risk]
    The excess risk on the test distribution is \yiping{If this definition is fine?}
    \begin{equation*}
        % E(G_1, G_2) = \E_{
        %     (\vx_i^{(1)},\vx_i^{(2)}), (\vx_j^{(1)},\vx_j^{(2)}) \sim \mathcal{P}^{te}_{X^2}
        % }[(s_{ij} - s^*_{ij})^2]
        ER(G_1, G_2) = \frac{1}{2}\E_{
            \vw_i, \vw_j\sim \mathcal{P}^{te}_{X^2}
        }\left[(s_{ij} - s^*_{ij})^2 + (s_{ji} - s^*_{ji})^2\right]
    \end{equation*}
\end{definition}
Then if we choose $\rho = n/(n-1)$, and note that the data generation for the two modality are symmetric, and thus $\Gamma$ is symmetric with high probability, then we can obtain
\begin{equation}\label{eq:ERapprox}
    ER(\hat G_1, \hat G_2) \approx 
    \mathop{\E}_{\vw_i, \vw_j\sim \mathcal{P}^{te}_{X^2}} [(\vy_i^{(1)})^\top (\Gamma - I_r)\vy_j^{(2)}]^2 
\end{equation}
% where $\vy^{(l)}$ is defined in Lemma~\ref{lemma:EYM}. 
Then from (\ref{eq:ERapprox}), we know that minimize the absolute value of the terms in the top left block of matrix $\Gamma - I_r$ will be more important than others because those terms corresponding to more frequently sampled features.

\yiping{TODO: Add another measurement to mimic imagenet classification error. Show that balance class can still be beneficial by maximize the cond}

\yiping{Maybe the results can be generalized to the case where the features of \textbf{downstream tasks} are give?}
\section{}

\fi



\iffalse
Define $\vx, \vy \in \R^d$ be the image and text inputs, and $\hat f, \hat g : \R^d \rightarrow \R^r$ as the image and text encoders, respectively. And we use $\vf_i := \hat{f}(\vx_i)/\|\hat{f}(\vx_i)\|_2$ to denote the normalized embedding for the $i$-th image inputs, and similar notation for $\vg_i$. Further let $\alpha_{ij} = \vf_i^\top \vg_j$ be the pairwise cosine similarity and $\beta_{ij} = \exp(\alpha_{ij}/\tau)$ be its exponentiation of with fixed temperature parameter $\tau$. Then we can then write the CLIP loss as
\begin{equation}\label{eq:CLIPloss}
    \mathcal{L} = -\frac{\tau}{2}\sum_{i=1}^n\left[\log(\frac{\beta_{ii}}{\sum_{j=1}^n\beta_{ij}})+\log(\frac{\beta_{ii}}{\sum_{j=1}^n\beta_{ji}})\right]
\end{equation}
We assume that the multi-modal data is generated by two different linear mapping with the same latent variables $\vz \in \R^r$, i.e.,
\begin{equation}
    \vx = F^* (\vz + \vvxi^{x}), \quad \vy = G^* (\vz + \vvxi^{y})
\end{equation}
where $F^*, G^* \in O_{d\times r}$ has orthonormal columns and $\vvxi^x, \vvxi^y \sim \mathcal{N}(0, \sigma^2 I_r), \sigma \ll 1$ are independent random noise. This assumption is widely used in previous works~\cite{XXX}.
Further, we use linear model  $\hat f(\vx) := \hat F^\top\vx, \hat g(\vy) := \hat G^\top\vy$ where $\hat F, \hat G \in \R^{d\times r}$, to minimize the contrastive loss. We use stochastic gradient descent with all the data in a batch to update the parameters, i.e., 
\begin{equation*}
    \hat F(t+1) = \hat F(t) - \frac{\eta}{n}\sum_{i=1}^n \vx_i(\left.\frac{\partial \mathcal{L}}{\partial \hat f(\vx_i)}\right|_t)^\top
\end{equation*}
\begin{equation*}
    \hat G(t+1) = \hat G(t) - \frac{\eta}{n}\sum_{i=1}^n \vy_i(\left.\frac{\partial \mathcal{L}}{\partial \hat g(\vy_i)}\right|_t)^\top
\end{equation*}

\section{Main Motivation}
We must mention that \emph{minimizing (\ref{eq:CLIPloss}) doesn't mean learning the ground truth head $F^*, G^*$}.
A simple example is  considering the case with $n=r$ samples for training, where $\vz_i = \ve_i, i \in [r-1]$ and $\vz_r = (1-\varepsilon)\ve_{r-1} + \varepsilon\ve_r$, $\varepsilon \ll 1$. It's clear that if $\hat F = F^*, \hat G = G^*$, we will have $\beta_{r-1,r}, \beta_{r,r-1}\approx \beta_{r-1,r-1}$, which means that $r-1$-th and $r$-th samples are confusing to the model. However, we can always find some rank-$r$ linear matrix $(\hat F)^\top F^*, (\hat G)^\top G^*$ to map any $r$ vectors onto $r$ orthogonal vectors, which means the learner $\hat F, \hat G$ can separate all the samples well and further minimize the CLIP loss. \yifang{I think it would be better to clearly define what is a good representation ? For example, previous work define a bad representation by saying under all possible linear classifier (the linear head), it is impossible to get good acc.}
\yiping{Yes, intuitionally the repr function that maps the input from different classes into a more separate space will have better downstream performance. I will add it soon. }

Following this observation, our motivation is that not all the classes are evenly distributed in the embedding space generated by the OpenAI CLIP model.\yiping{Need visualization}. Classes with many similar features are always generated by close latent variables, which will result in similar embeddings and take a much longer time for the learners to separate each other. This can happen even when the image and text encoders are perfectly aligned.

\begin{assumption}[Data Classes]\label{ass:classes}
Assume we have $r$ different classes and the sample number in the $i$-th class is $n_i$, so $n = \sum_i^r n_i$. The classes are determined by $r$ different latent variables $\{\bar\vz_{i}\}_1^{r}$ satisfies:  $\bar\vz_r := (1-\varepsilon)\bar\vz_{r-1} + \varepsilon\bar\vz'$, $\{\bar\vz_1, \ldots, \bar\vz_{r-1}, \bar\vz'\}$ are orthonormal vectors.
\end{assumption}
\begin{theorem}
    \yiping{Need further calculation}(Informal) Assume Assumption~\ref{ass:classes} holds with parameters $\{n_i\}_1^r, \varepsilon$. Then if $\hat F(0)^\top F^* \approx \hat G(0)^\top G^*$\yiping{This assumption should not be necessary}, we claim that $\hat F(t)^\top F^*\approx \hat G(t)^\top G^*$, $\alpha_{r,r-1}, \alpha_{r-1,r}$ decreasing in the rate of $O(\varepsilon\cdot(n_{r-1}+n_{r})/{n})$, while for all other $\alpha_{i,j}, i\neq j$, their decreasing rate is $O((n_{i}+n_{j})/{n})$
\end{theorem}

\yiping{Add class definition. $n_i$ is the number of samples for class $i$.}
\fi



% Acknowledgements should only appear in the accepted version.
% \section*{Acknowledgements}

% \textbf{Do not} include acknowledgements in the initial version of
% the paper submitted for blind review.

% If a paper is accepted, the final camera-ready version can (and
% probably should) include acknowledgements. In this case, please
% place such acknowledgements in an unnumbered section at the
% end of the paper. Typically, this will include thanks to reviewers
% who gave useful comments, to colleagues who contributed to the ideas,
% and to funding agencies and corporate sponsors that provided financial
% support.


% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite

% \nocite{langley00}

